Insights from Generative Modeling for Neural Video Compression

While recent machine learning research has revealed connections between deep generative models such as VAEs and rate-distortion losses used in learned compression, most of this work has focused on images. In a similar spirit, we view recently proposed neural video coding algorithms through the lens of deep autoregressive and latent variable modeling. We present these codecs as instances of a generalized stochastic temporal autoregressive transform, and propose new avenues for further improvements inspired by normalizing flows and structured priors. We propose several architectures that yield state-of-the-art video compression performance on high-resolution video and discuss their tradeoffs and ablations. In particular, we propose (i) improved temporal autoregressive transforms, (ii) improved entropy models with structured and temporal dependencies, and (iii) variable bitrate versions of our algorithms. Since our improvements are compatible with a large class of existing models, we provide further evidence that the generative modeling viewpoint can advance the neural video coding field.

==> OLD.tex <==
\begin{table*}[ht]
\centering
\caption{\textbf{Overview of compression methods and the datasets trained on} (if applicable).}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Model Name}   & \textbf{Category} & \textbf{Vimeo-90k} & \textbf{Youtube-NT} & \textbf{Remark}                                                                              \\
\hline\hline
\textbf{STAT-SSF}       & Proposed & \cmark         & \cmark          & Proposed autoregressive transform with scale space flow                       \\
\hline
\textbf{STAT-SSF-SP}    & Proposed & \cmark         & \xmark          & Same as above (STAT-SSF) but with structured prior \\
\hline
\textbf{STAT-SSF-SP-TP+}    & Proposed & \cmark & \xmark &  \makecell{Structured prior and improved temporal prior, $p(\bv_t|\hatx_{t-1}, \w_t)$}\\
\hline
\hline
SSF          & Baseline & \cmark         & \cmark          & Agustsson et al.\cite{agustsson2020scale}                                 \\
\hline
DVC          & Baseline & \cmark         & \xmark          & Lu et al.\cite{lu2019dvc}                                                                 \\
\hline
VCII    & Baseline & \xmark       & \xmark        & Wu et al.\cite{wu2018video} (trained on the Kinectics dataset)                                            \\
\hline
DGVC         & Baseline & \cmark         & \xmark          & Han et al.\cite{han2018deep} modified for low-latency compression setup                                                        \\
\hline
TAT          & Baseline & \cmark         & \xmark          & Yang et al.\cite{yang2020autoregressive}                                                    \\
\hline
HEVC    & Baseline & N/A       & N/A        & FFMPEG-HEVC with RGB 4:4:4 color space input                                            \\
\hline
HEVC(YUV)    & Baseline & N/A       & N/A        & FFMPEG-HEVC with YUV 4:2:0 color space input                                         \\
\hline
STAT         & Ablation & \cmark         & \cmark          & STAT-SSF without optical flow   \\
\hline
SSF-SP       & Ablation & \xmark         & \cmark          & SSF with structured prior                                       \\
\hline
SSF-TP    & Ablation & \cmark & \xmark & SSF with temporal prior conditioned on $\bv_{t-1}$, $p(\bv_t|\bv_{t-1})$\\
\hline
SSF-TP+    & Ablation & \cmark & \xmark & SSF with temporal prior conditioned on $\hatx_{t-1}$,  $p(\bv_t|\hatx_{t-1})$\\
\hline
\end{tabular}
}
\label{tab:table-model}
\end{table*}


As we saw above, normalizing flow models implement the key idea of transform coding -- finding a simplified, and typically factorized representation of the data where scalar quantization can be fruitfully applied. However, the learned model does not take into account the subsequent quantization, and the final decoded representations $\hatx$ can have uncontrolled distortion. 
Rather than viewing quantization and entropy coding as a separate, post-hoc procedure,  end-to-end compression with variational autoencoders \cite{balle2017end, theis2017lossy, balle2020nonlinear} jointly optimize all components of transform coding in order to achieve optimal rate-distortion performance.

To motivate this approach, consider transform coding with a pair of flexible (but not necessarily invertible) transforms $f$  (``encoder'') and $g$ (``decoder'') that map between the video $\x_{1:T}$ and its transformed representation $\barz_{1:T} = f(\x_{1:T})$. Given sufficiently expressive $f$ and $g$,  quantization can be performed by element-wise rounding to the nearest integer, $\round{\cdot}$, resulting in the following R-D objective,
\begin{align}
\mathcal{L} = \mathbb{E}_{\x_{1:T} \sim p_\text{data}}[ \mathcal{D}(\x_{1:T}, g(\round{f(\x_{1:T})})) + \beta \mathcal{R}(\round{ f(\x_{1:T}) }) ].
\end{align}
Following \cite{balle2017end},
we approximate the rounding operations
by uniform noise injection to enable gradient-based optimization during training.
The resulting, relaxed version of the above R-D objective can be shown to be equal to the expected Negative Evidence Lower BOund (NELBO) of a particular \emph{compressive VAE} model, described below \cite{balle2017end,theis2017lossy}:
\begin{multline}
    \tilde{\mathcal{L}} = \mathbb{E}_{\x_{1:T} \sim p_\text{data}}[ \mathbb{E}_{q(\z_{1:T}|\x_{1:T})} [ -\log p(\x_{1:T} | \z_{1:T} )
    \\
     -\log p(\z_{1:T}) ] ]. \label{eq:overall-nelbo}
\end{multline}
In this compressive VAE model, the approximately quantized representation $\round{\barz_{1:T}} \approx \barz_{1:T} + \mathbf{u}_{1:T},  \mathbf{u}_{1:T} \sim \mathcal{U}(-
\textbf{0.5}, \textbf{0.5})$ is associated with a sequence of latent variables $\z_{1:T}$ under a particular variational posterior distribution $q(\z_{1:T}|\x_{1:T}) = \mathcal{U}(\barz_{1:T}-0.5, \barz_{1:T}+0.5)$, i.e., a unit-width uniform distribution whose mean $\barz_{1:T}$ is predicted by an amortized inference network $f$, and has zero differential entropy. 
The likelihood $p(\x_{1:T}|\z_{1:T})$ follows a Gaussian distribution with fixed diagonal covariance  $\tfrac{\beta}{2 \log 2}  \mathbf{I}$, and mean $\hatx_{1:T} = g(\z_{1:T})$ computed by the generative network $g$, so that the negative log-likelihood $-\log p(\x_{1:T} | \z_{1:T} )$ equals the squared error distortion $\tfrac{1}{\beta} \|\x_{1:T} -\hatx_{1:T} \|^2$
weighted by $\tfrac{1}{\beta}$.
Following \cite{balle2017end}, the prior density $p(\z_{1:T})$ is parameterized to interpolate its discretized version $P(\z_{1:T})$, so that given integer valued $\z_{1:T}$, the negative log density $-\log p(\z_{1:T})$ measures the code length $-\log P(\z_{1:T})$ assigned by the entropy model $P ({\z_{1:T}})$. By minimizing the approximate R-D objective of Eq.~\ref{eq:overall-nelbo} with respect to the parameters of $f$, $g$, and $p( \z_{1:T})$, training an end-to-end neural compression model is thus equivalent to learning a VAE by maximum-likelihood and amortized variational inference. %
Note this is in contrast to the maximum-likelihood estimation of a normalizing flow model, which does not have the interpretation of an (approximate) R-D objective of lossy compression. The normalizing flow objective in Eq.~\ref{eq:flow-duality} can be interpreted as a degenerate case of the NELBO objective of a deterministic latent variable model, where there is no noise in the data generation or inference/quantization process, %
i.e., $q(\z_{1:T}|\x_{1:T}) = \delta_{F^{-1}(\x_{1:T})}(\z_{1:T})$ is a Dirac delta distribution concentrated on the encoding $F^{-1}(\x_{1:T})$, similarly $ p(\x_{1:T}|\z_{1:T}) = \delta_{F(\z_{1:T})}(\x_{1:T})$. Indeed, we note that normalizing flows have been succesfully applied to \emph{lossless} compression, where the expected negative log-likeilhood loss serves as an upper bound on the lossless data compression cost under a discretized entropy model \cite{ho2019compression}.

Given a compressive VAE, the compression of a data sequence $\x_{1:T}$ via transform coding closely corresponds to an inference-generation pass through the VAE, described in the following steps.
\textbf{1. encoding:} The encoder passes $\x_{1:T}$ through $f$ to obtain a transformed representation $\barz_{1:T}=f(\x_{1:T})$, thus computing the mean parameters $\barz_{1:T}$ of the variational distribution $q(\x_{1:T}|\z_{1:T})$ by amortized variational inference; \textbf{2. quantization and entropy coding:} A posterior sample $\z_{1:T}$ is drawn, i.e., $\z_{1:T} \sim q(\z_{1:T}|\x_{1:T})$ (or, deterministically computed as $\z_{1:T} = \round{\barz_{1:T}}$ at test time), and a bit-string encoding $\boldsymbol{\xi}$ of $\z_{1:T}$ is transmitted under the entropy model $P({\z_{1:T}})$; \textbf{3. decoding:} The decoder decodes $\z_{1:T}$ from bit-string $\boldsymbol{\xi}$ using the entropy model $P({\z_{1:T}})$, then computes the reconstruction by $\hatx_{1:T}=g(\z_{1:T})$, corresponding to the mean parameters of the Gaussian likelihood model $p( \x_{1:T}| \z_{1:T})$. Note that step 3 (decoding) is analogous to sampling from the generative model, but without adding diagonal Gaussian noise to $\hatx_{1:T}$ dictated by the Gaussian likelihood $p( \x_{1:T}| \z_{1:T})$. Indeed, if the bit-string  $\boldsymbol{\xi}$ consists of a sequence of purely random bits, then it is well known that decoding $\boldsymbol{\xi}$ under the entropy model $P({\z_{1:T}})$ produces a sample  $\z_{1:T} \sim P({\z_{1:T}})$ \cite{cover1999elements}. For this reason, in the following discussions we occasionally blur the distinction between the (random) latent variable $\z_{1:T} \sim P({\z_{1:T}})$ and the quantized latent representation $\round{\barz_{1:T}}$ (as would be decoded from a bitstring $\boldsymbol{\xi}$) to simplify notation. 

A data compression process with such a learned transform coding algorithm also implicitly defines a VAE model for the data. Specifically, let us consider the compression procedure of an online video compression codec, in which individual frames $\x_t$ are transmitted in sequence without the knowledge of future frames $\x_{>t}$.
The encoding-decoding process is specified recursively as follows.
Given the ground truth current frame $\x_t$ and the previously reconstructed frames $\hatx_{<t}$, the encoder is restricted to be of the form $\barz_t = f(\x_t,\hatx_{<t})$, and similarly the decoder computes reconstruction sequentially based on previous reconstructions and the current encoding, $\hatx_t = g(\hatx_{<t}, \round{\barz_t}))$. Existing codecs usually condition on a \emph{single} reconstructed frame, substituting $\hatx_{<t}$ by $\hatx_{t-1}$ in favor of efficiency.
In the language of generative modeling and variational inference, the sequential encoder corresponds to a variational posterior of the form $q(\z_t|\x_t, \z_{<t})$, i.e., filtering,
and the sequential decoder corresponds to the likelihood $p(\x_t|\z_{\leq t})=\mathcal{N}(\hatx_t, \tfrac{\beta}{2\log 2}  \mathbf{I})$;  in both distributions, the probabilistic conditioning on $\z_{<t}$ is based on the observation that $\hatx_{t-1}$ is a deterministic function of $\z_{<t}$, if we identify $\round{ \barz_{t} }$ with the random variable $\z_{t}$ and unroll the recurrence $\hatx_t = g(\hatx_{<t}, \z_{t})$.  As we show, all sequential compression approaches considered in this work follow this paradigm, and implicitly define generative models of the data as $ p(\x_{1:T}) \propto  p(\x_{1:T} | \z_{1:T}) p(\z_{1:T}) = p(\z_{1:T}) \prod_t p(\x_t | \z_{\leq t})$, where the likelihood model $p(\x_t | \z_{\leq t})$ at each time step is centered on the reconstruction $\hatx_t$. The key difference is in the definition of the decoding transform for computing $\hatx_t$ as a (stochastic) function of $\hatx_{<t}$ and $\z_t$.




==> method.tex <==
\section{Video Compression through Deep Autoregressive Modeling}

We identify commonalities between hierarchical autoregressive flow models \cite{marino2020improving} and state-of-the-art neural video compression architectures \cite{agustsson2020scale}, and will use this viewpoint to propose improvements on existing models. 

\subsection{Background}\label{sec:background}
We first review VAE-based compression schemes \cite{balle2017end} and formulate existing low-latency video codecs in this framework; we then review
the related autoregressive flow model. 

\textbf{Generative Modeling and Source Compression.} 
Given a a sequence of video frames $\x_{1:T}$, lossy compression seeks a compact description of  $\x_{1:T}$ that simultaneously minimizes the description length $\mathcal R$ and information loss $\mathcal D$.
The distortion~$\mathcal D$ measures the reconstruction error caused by encoding $\x_{1:T}$
into a lossy representation $\bar{\z}_{1:T}$ and
subsequently decoding it back to $\hatx_{1:T}$, while~$\mathcal R$ measures the bit rate (file size).
In learned compression methods \cite{balle2017end, theis2017lossy}, the above process is parameterized by flexible functions $f$  (``encoder'') and $g$ (``decoder'') that map between the video and its latent representation $\barz_{1:T} = f(\x_{1:T})$.
The goal is to minimize a rate-distortion loss, with the tradeoff between the two controlled by a hyperparameter $\beta>0$:
\[
\mathcal{L} = \mathcal{D}(\x_{1:T}, g(\round{\barz_{1:T}})) + \beta \mathcal{R}(\round{ \barz_{1:T} }).
\]
We adopt the end-to-end compression approach of \cite{balle2017end}, which approximates the rounding operations $\round{\cdot}$ (required for entropy coding) by uniform noise injection to enable gradient-based optimization during training.
With an appropriate choice of probability model $p(\z_{1:T})$, the relaxed version of above R-D (rate-distortion) objective then corresponds to the VAE objective:
\begin{align}
    \tilde{\mathcal{L}} = \mathbb{E}_{q(\z_{1:T}|\x_{1:T})} [ -\log p(\x_{1:T} | \z_{1:T} ) - \log p(\z_{1:T})  ] . \label{eq:overall-nelbo}
\end{align}
In this model, the likelihood $p(\x_{1:T}|\z_{1:T})$ follows a Gaussian distribution with mean $\hatx_{1:T} = g(\z_{1:T})$ and diagonal covariance  $\tfrac{\beta}{2 \log 2}  \mathbf{I}$, 
and the approximate posterior $q$ is chosen to be a unit-width uniform distribution (thus has zero differential entropy) whose mean $\barz_{1:T}$ is predicted by an amortized inference network $f$. The prior density $p(\z_{1:T})$ interpolates its discretized version, so that it measures the code length of discretized $\barz_{1:T}$ after entropy-coding. 

\textbf{Low-Latency Sequential Compression}
We specialize Eq.~\ref{eq:overall-nelbo} to make it suitable for low-latency video compression, widely used in both conventional and recent neural codecs \cite{Rippel2019LearnedVC, agustsson2020scale}. 
To this end, we encode and decode individual frames $\x_t$ in sequence. 
Given the ground truth current frame $\x_t$ and the previously reconstructed frames $\hatx_{<t}$, the encoder is restricted to be of the form $\barz_t = f(\x_t,\hatx_{<t})$, and similarly the decoder computes reconstruction sequentially based on previous reconstructions and the current encoding, $\hatx_t = g(\hatx_{<t}, \round{\barz_t}))$. Existing codecs usually condition on a \emph{single} reconstructed frame, substituting $\hatx_{<t}$ by $\hatx_{t-1}$ in favor of efficiency.
In the language of variational inference, the sequential encoder corresponds to a variational posterior of the form $q(\z_t|\x_t, \z_{<t})$, i.e., filtering,
and the sequential decoder corresponds to the likelihood $p(\x_t|\z_{\leq t})=\mathcal{N}(\hatx_t, \tfrac{\beta}{2\log 2}  \mathbf{I})$;  in both distributions, the probabilistic conditioning on $\z_{<t}$ is based on the observation that $\hatx_{t-1}$ is a deterministic function of $\z_{<t}$, if we identify $\round{ \barz_{t} }$ with the random variable $\z_{t}$ and unroll the recurrence $\hatx_t = g(\hatx_{<t}, \z_{t})$. As we show, all sequential compression approaches considered in this work follow this paradigm, and the form of the reconstruction transform $\hatx$ determines the lowest hierarchy of the corresponding generative process of video $\x$.


\textbf{Masked Autoregressive Flow (MAF).}
As a final component in neural sequence modeling, we discuss MAF \cite{papamakarios2017masked}, which models the joint distribution of a sequence $p(\x_{1:T})$ in terms of a simpler distribution of its underlying noise variables $\y_{1:T}$ through the following autoregressive transform and its inverse:
\begin{align}
    \x_t = h_\mu(\x_{<t}) + h_\sigma(\x_{<t}) \odot \y_t; \; \Leftrightarrow \; 
    \y_t = \textstyle{\frac{\x_t - h_\mu(\x_{<t})} {h_\sigma(\x_{<t})}}.
    \label{eq:MAF}
\end{align}
The noise variable $\y_t$ usually comes from a standard normal distribution. While the forward MAF transforms a sequence of standard normal noises into a data sequence, the inverse flow ``whitens'' the data sequence and removes temporal correlations. Due to its invertible nature, MAF allows for exact likelihood computations, but as we will explain in Section~\ref{sec:models}, we will not exploit this aspect in compression but rather draw on its expressiveness in modeling conditional likelihoods.

\subsection{A General Framework for Generative Video Coding}\label{sec:method-stat}
We now describe a general framework that captures several existing low-latency neural compression methods as specific instances and gives rise to the exploration of new models. To this end, we combine latent variable models with autoregressive flows into a joint framework. We consider a sequential decoding procedure of the following form: 
\begin{align}
    \hatx_t = h_\mu(\hatx_{t-1}, \w_t) + h_\sigma(\hatx_{t-1}, \w_t) \odot g_v(\bv_t, \w_t).
    \label{eq:master}
\end{align}
Eq.~\ref{eq:master} resembles the definition of the MAF in Eq.~\ref{eq:MAF}, but augments this transform with two sets of latent variables $\w_t,\bv_t \sim p(\w_t,\bv_t)$. Above, $h_\mu$ and $h_\sigma$ are functions that transform the previous reconstructed data frame $\hatx_{t-1}$ along with $\w_t$ into
a shift and scale parameter, respectively. The function $g_v(\bv_t, \w_t)$ converts these latent variables into a noise variable that encodes residuals with respect to the mean next-frame prediction $h_\mu(\hatx_{t-1}, \w_t)$.

This stochastic decoder model has several advantages over existing generative models for compression, such as simpler flows or sequential VAEs. First, the stochastic autoregressive transform $h_\mu(\hatx_{t-1}, \w_t)$ involves a latent variable $\w_t$ and is therefore more expressive than a deterministic transform \cite{schmidt2018deep,schmidt2019autoregressive}.
Second, compared to MAF, the additional nonlinear transform $g_v(\bv_t, \w_t)$ enables more expressive residual noise, reducing the burden on the entropy model. Finally, as visualized in Figure~\ref{fig:qulitative-scale}, the scale parameter $h_\sigma(\hatx_{t-1}, \w_t)$ effectively acts as a gating mechanism, determining how much variance is explained in terms of the autoregressive transform and the residual noise distribution. This provides an added degree of flexibility, in a similar fashion to  how RealNVP improves over NICE \cite{dinh2014nice, dinh2016density}.

Our approach is inspired by \cite{marino2020improving} who analyzed a  restricted version of the model in Eq.~\ref{eq:master}, aiming to hybridize autoregressive flows and sequential latent variable models for video prediction. In contrast to Eq.~\ref{eq:master}, their model involved deterministic transforms  as well as residual noise that came from a sequential VAE.
\subsection{Example Models and Extensions}\label{sec:models}

Next, we will show that the general framework expressed by Eq.~\ref{eq:master} captures a variety of state-of-the-art neural video compression schemes and gives rise to extensions and new models. 

\textbf{Temporal Autoregressive Transform (TAT).}
The first special case among the class of models that are captured by Eq.~\ref{eq:master} is the autoregressive neural video compression model by \cite{yang2020autoregressive}, which we refer to as temporal autoregressive transform (TAT). Shown in Figure \ref{fig:model-diagram}(a), the decoder $g$ implements a deterministic scale-shift autoregressive transform of decoded noise $\y_t$,
\begin{align}
    \hatx_t = g(\z_t, \hatx_{t-1}) = h_\mu(\hatx_{t-1}) + h_\sigma(\hatx_{t-1}) \odot \y_t, \quad \y_t = g_z(\z_t).
    \label{eq:decoder-tat}
\end{align}
The encoder $f$ inverts the transform to decorrelate the input frame $\x_t$ into $\bary_t$ and encodes the result as $\barz_t = f(\x_t,\hatx_{t-1}) = f_z(\bary_t)$, where $\bary_t =\frac{\x_t -h_\mu(\hatx_{t-1})}{h_\sigma(\hatx_{t-1})}$. The shift $h_\mu$ and  scale $h_\sigma$ transforms are parameterized by neural networks, $f_z$ is a convolutional neural network (CNN), and $g_z$ is a deconvolutional neural network (DNN) that approximately inverts $f_z$.

The TAT decoder is a simple version of the more general stochastic autoregressive transform in Eq~\ref{eq:master}, where $h_\mu$ and $h_\sigma$ lack latent variables.
Indeed, interpreting the probabilistic generative process of $\hatx$, TAT implements the model proposed by \cite{marino2020improving}, as the transform from $\y$ to $\hatx$ is a MAF. However, the generative process corresponding to compression (reviewed in Section~\ref{sec:background}) adds additional white noise to $\hatx$, with $\x:=\hatx + \boldsymbol{\epsilon}, \boldsymbol{\epsilon}\sim \mathcal{N}(\mathbf{0}, \tfrac{\beta}{2\log 2} \mathbf{I})$. Thus, the generative process from $\y$ to $\x$ is no longer an autoregressive flow.
Regardless, TAT was shown to better capture the low-level dynamics of video frames than the autoencoder $(f_z, g_z)$ alone, and the inverse transform decorrelates raw video frames to simplify the input to the encoder $f_z$ \cite{yang2020autoregressive}.



\begin{figure*}[t!]
    \centering
    \includegraphics[width=.6\linewidth]{figs/iclr2021-models-highlighted-crop.pdf}
    \caption{\textbf{Model diagrams} for the generative and inference procedures of the current frame $\x_t$, for various neural video compression methods. Random variables are shown in circles, all other quantities are deterministically computed; solid and dashed arrows describe computational dependency during generation (decoding) and inference (encoding), respectively. Purple nodes correspond to neural encoders (CNNs) and decoders (DNNs), and green nodes implement temporal autoregressive transform.
    (a) TAT; (b) SSF; (c) STAT or STAT-SSF; the magenta box highlights the additional proposed scale transform absent in SSF, and the red arrow from $\w_t$ to $\bv_t$
    highlights the proposed (optional) structured prior. 
    See Appendix Fig. \ref{fig:archi} for computational diagrams of the structured prior.
    }
    \label{fig:model-diagram}
\end{figure*}


\textbf{DVC \cite{lu2019dvc} and Scale-Space Flow (SSF, \cite{agustsson2020scale}).}
The second class of models captured by Eq.~\ref{eq:master} belong to the conventional video compression framework based on predictive coding \cite{cutler1952differential, wiegand2003overview, sullivan2012overview}; both models make use of two sets of latent variables $\z_{1:T} = \{ \w_{1:T}, \bv_{1:T}  \}$ to capture different aspects of information being compressed,
where $\w$ captures estimated motion information used in warping prediction, and $\bv$ helps capture residual error not predicted by warping.  

Like most classical approaches to video compression by predictive coding, the reconstruction transform in the above models has the form of a prediction shifted by residual error (decoded noise), and lacks the scaling factor $h_\sigma$ compared to the autoregressive transform in Eq.~\ref{eq:master}
\begin{align}
    \hatx_t = h_{warp}(\hatx_{t-1}, g_w(\w_t)) + g_v(\bv_t, \w_t). \label{eq:encoder-ssf}
\end{align}
Above, $g_w$ and $g_v$ are DNNs, $\mathbf{o}_t := g_w(\w_t)$ has the interpretation of an estimated optical flow (motion) field, $h_{warp}$ is the computer vision technique of warping, 
and the residual $\br_t := g_v(\bv_t, \w_t) = \hatx_t - h_{warp}(\hatx_{t-1}, \mathbf{o}_t)$ represents the prediction error unaccounted for by warping.
\cite{lu2019dvc} only makes use of $\bv_t$ in the residual decoder $g_v$, and performs simple 2D warping by bi-linear interpretation;
SSF \cite{agustsson2020scale} augments the optical flow (motion) field $\mathbf{o}_t$ with an additional scale field,
and applies scale-space-warping to the progressively blurred versions of $\hatx_{t-1}$ to allow for uncertainty in the warping prediction.
The encoding procedure in the above models compute the variational mean parameters as $\barw_t = f_w(\x_t, \hatx_{t-1}), \barv_t = f_v(\x_t - h_{warp}(\hatx_{t-1}, g_w(\w_t)))$, corresponding to a structured posterior $q(\z_t | \x_t, \z_{<t}) = q(\w_t| \x_t, \z_{<t}) q(\bv_t| \w_t, \x_t, \z_{<t})$.  We illustrate the above generative and inference procedures in Figure~\ref{fig:model-diagram}(b).

\textbf{Proposed: models based on Stochastic Temporal Autoregressive Transform.}
Finally, we consider the most general models as described by the stochastic autoregressive transform in Eq.~\ref{eq:master}, shown in Figure~\ref{fig:model-diagram}(c).
We study two main variants, categorized by how they implement $h_\mu$ and $h_\sigma$:
\begin{itemize}
    \item \textbf{STAT} uses DNNs for $h_\mu$ and $h_\sigma$ as in (Yang et al., 2020b), but complements it with the latent variable $\w_t$ that characterizes the transform. In principle, more flexible transforms should give better compression performance, but we find the following variant more parameter efficient in practice:
    
    \item \textbf{STAT-SSF}: a less data-driven variant of the above that still uses scale-space warping \cite{agustsson2020scale} in the shift transform, i.e., $h_\mu(\hatx_{t-1}, \w_t) = h_{warp}(\hatx_{t-1}, g_w(\w_t))$. This can also be seen as an extended version of the SSF model, whose shift transform $h_\mu$ is preceded by a new learned scale transform $h_\sigma$.
\end{itemize}

\textbf{Structured Prior (SP). }
Besides improving the autoregressive transform (affecting the likelihood model for $\x_t$), one variant of our approach also improves the topmost generative hierarchy in the form of a more expressive latent prior $p(\z_{1:T})$, affecting the entropy model for compression. We observe that motion information encoded in $\w_t$ can often be informative of the residual error encoded in $\bv_t$. In other words, large residual errors $\bv_t$ incurred by the mean prediction $h_\mu(\hatx_{t-1}, \w_t)$ (e.g., the result of warping the previous frame $h_\mu(\hatx_{t-1}$)) are often spatially collocated with (unpredictable) motion as encoded by $\w_t$.

The original SSF model's prior factorizes as $p(\w_t, \bv_t) = p(\w_t) p(\bv_t)$ and does not capture such correlation. 
We therefore propose a structured prior by introducing conditional dependence between $\w_{t}$ and $\bv_t$, so that $ p(\w_t, \bv_t) =  p(\w_t) p(\bv_t | \w_t)$. At a high level, this can be implemented by introducing a new neural network that maps $\w_t$ to parameters of a parametric distribution of $p(\bv_t | \w_t)$ (e.g., mean and variance of a diagonal Gaussian distribution).
This results in variants of the above models, \textbf{STAT-SP} and \textbf{STAT-SSF-SP}, where the structured prior is applied on top of the proposed \textbf{STAT} and \textbf{STAT-SSF} models.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=1\linewidth]{figs/vis-ssf-dep-af-st-SND-beta=0.000625.pdf}
    \caption{\textbf{Visualizing the proposed STAT-SSF-SP model} on one frame of UVG video ``Shake-NDry''. 
    Two methods in comparison, STAT-SSF (proposed) and SSF \cite{agustsson2020scale}, have comparable reconstruction quality to STAT-SSF-SP but higher bit-rate; the (BPP, PSNR) for STAT-SSF-SP, STAT-SSF, and SSF are (0.046, 36.97), (0.053, 36.94), and (0.075, 36.97), respectively.
    In this example, the warping prediction $\bm{\hat\mu}_t = h_\mu(\hatx_{t-1}, \round{\barw_t})$ incurs large error around the dog's moving contour, but models the mostly static background well, with the residual latents $\round{\barv_t}$ taking up an order of magnitude higher bit-rate than $\round{\barw_t}$ in the three methods.
    The proposed scale parameter $\bm{\hat\sigma}_t$ gives the model extra flexibility when combining the noise $\haty_t$ (decoded from $(\round{\barv_t}, \round{\barw_t})$) with the warping prediction $\bm{\hat\mu}_t$ (decoded from $\round{\barw_t}$ only) to form the reconstruction $\hatx_t = \bm{\hat\mu}_t + \bm{\hat\sigma}_t \odot \haty_t$: the scale $\bm{\hat\sigma}_t$ downweights contribution from the noise $\haty_t$ in the foreground where it is very costly, and reduces the residual bit-rate $\mathcal{R}(\round{\barv_t})$ (and thus the overall bit-rate) compared to STAT-SSF and SSF (with similar reconstruction quality), as illustrated in the third and fourth figures in the top row.
    }
    \label{fig:qulitative-scale}
\end{figure*}

